A Parameterized Perspective on Protecting Elections

We study the parameterized complexity of the optimal defense and optimal attack problems in voting. In both the problems, the input is a set of voter groups (every voter group is a set of votes) and two integers $k_a$ and $k_d$ corresponding to respectively the number of voter groups the attacker can attack and the number of voter groups the defender can defend. A voter group gets removed from the election if it is attacked but not defended. In the optimal defense problem, we want to know if it is possible for the defender to commit to a strategy of defending at most $k_d$ voter groups such that, no matter which $k_a$ voter groups the attacker attacks, the outcome of the election does not change. In the optimal attack problem, we want to know if it is possible for the attacker to commit to a strategy of attacking $k_a$ voter groups such that, no matter which $k_d$ voter groups the defender defends, the outcome of the election is always different from the original (without any attack) one.

==> pseudo_scoring_defense.tex <==
The proof is based on dynamic programming algorithm. Let  $(\CC, \{\GG_i: i\in[n]\}, k_a, k_d)$ be an instance of the $r$-\OD problem, and suppose $|\CC| = m+1$. In particular, let $\CC = \{c_0, c_1, \ldots, c_m\}$, and let $c_0$ be the winner of the election, that is, let $c_0 = r(\{\GG_i\}_{i\in[n]})$. Further, $X := \{-N, -(N-1), \ldots, (N-1),N\}$, and let $\lambda \in X^m$ be a vector with $m$ coordinates. For $1 \leq i \leq m$, we use $\lambda[i]$ to refer to the $i^{th}$ coordinate of $\lambda$.  


For $i \in [n]$, $p \in [k_d]$, $q \in [k_a]$ and $\lambda \in X^m$, we define the function ${\mathcal D}(i,p,q,\lambda)$ as follows. Intuitively, we think of $\lambda$ as a ``demand vector'', and ${\mathcal D}$ represents the possibility of defending $p$ resources (among the first $i$ voter groups) in such a way that no matter which $q$-sized subset of the first $i$ voter groups are attacked, the score difference between $c_0$ and $c_i$ remains at least $\lambda[i]$ for all $1 \leq i \leq m$ in the resulting election. 

To formalize this, let us say that $i,p,q$ is \textit{good} with respect to $\lambda$ if there exists an index set $\II\subseteq [i]$ with $|\II|\le p$ such that, for every $\II^\pr\subset [i]\setminus\II$ with $|\II^\pr|\le q$, we have:

$$s_\GG(r,c_0) - s_\GG(r,c_i) \geq \lambda[i], \forall 1 \leq i \leq m,$$

where $s_\GG(r,x)$ denotes the score of the candidate $x$ using the scoring rule $r$ in the election $\{\GG_i: i\in[n]\}$. We now define ${\mathcal D}$ as follows:


\[ {\mathcal D}(i,p,q,\lambda) = \begin{cases} 1 &\mbox{if } i,p,q \mbox{ is good for } \lambda \\ 
0 & \mbox{otherwise. }\end{cases}  \]


We now have the following recurrence:

\[ {\mathcal D}(i,p,q,\lambda) =   {\mathcal D}(i-1,p,q,\lambda) \mbox{ OR } \left({\mathcal D}(i-1,p-1,q-1,\mu) \mbox{ AND } {\mathcal D}(i-1,p-1,q,\lambda)\right), \]
